A Decision Procedure for String Logic with Equations, Regular Membership and Length Constraints

In this paper, we consider the satisfiability problem for string logic with equations, regular membership and Presburger constraints over length functions. The difficulty comes from multiple occurrences of string variables making state-of-the-art algorithms non-terminating. Our main contribution is to show that the satisfiability problem in a fragment where no string variable occurs more than twice in an equation is decidable. In particular, we propose a semi-decision procedure for arbitrary string formulae with word equations, regular membership and length functions. The essence of our procedure is an algorithm to enumerate an equivalent set of solvable disjuncts for the formula. We further show that the algorithm always terminates for the aforementioned decidable fragment. Finally, we provide a complexity analysis of our decision procedure to prove that it runs, in the worst case, in factorial time.

==> algo-eql.tex <==



\begin{verbatim}
for each solution
  - add length constraint
  - decidable (solved form of
   \cite{Abdulla:CAV:2014})
\end{verbatim}

\cite{Abdulla:CAV:2014}


==> algo-regex.tex <==


\locsay{}


==> algo.tex <==
%%\input{sat-algo}
%% In this section, we present a decision procedure for checking
%% satisfiability of {\strel} formula with word equation, regular membership
%% and arithmetic on length functions.
%%%%%%%%%%%%%%%%%%%%%%%
%%  We start with
%% defining our target formulas. Let {\basetheory}
%% be a {\em base theory} (logic) with the following properties: (i)
%% {\basetheory} is closed under propositional combination and supports
%% boolean variables; (ii) there exists a complete decision procedure
%% for {\basetheory}. Let ${\basetheory}^{ind}$ be the extension of {\basetheory}
%% with inductive predicate instances defined in a system with a set of
%% predicates \form{\PName{=} \{P_1, ..., P_k \}}. Each predicate
%% may be annotated with a {\em sound} invariant.
%% We use \form{\base} to denote a formula in {\basetheory}
%% and \form{\ind} to denote a formula in the extended theory.
%% Semantically, \form{\ind{\equiv}\bigvee_{i{=}0}^n \base_i, ~ n{\geq}0}.
%%
Given a {\strel} formula \form{\pure},
we invoke function \code{reduce}
to obtain a generalized equation $\sge_0$
with size $\gesize{n}{m}$, i.e.
$ \code{reduce}(\pure) \yields \sge_0\gesize{n}{m}$.
After that, we invoke procedure  {\algoname} to decide
$\sge_0$.

{\algoname} is an instantiation of the generic algorithm
{\satalgo} presented in Algorithm \ref{algo.solved.sat}. %%\cite{Loc:CAV:2016}.
 In this instantiation,
 base formulas are those in {\solvedF}.
%% {\algoname} is presented in Algorithm~\ref{algo.s2.sat}.
%% {\algoname}  takes a {\strel} formula \form{\ind} as input,
%% it initially reduces this formula into a generalized equation {\sge}
%% and then iteratively derives unfolding trees for {\sge}.
%% By doing so, it systematically enumerates disjuntive set of \form{\sges}.
{\algoname} takes a generalized equation $\sge_0\gesize{n}{m}$
as input, iteratively derives unfolding trees for it
and
  can produce
two possible outcomes: {\sat} with a solution  %under-approximated 
 or {\unsat} with a proof.
%% We remark that nodes of these unfolding trees store
%% generalized equations.
In this subsection, we show how to instantiate 
functions \form{\code{init}_{\strel}}, {\uosea}, {\oosea}, \form{\code{prune\_out\_of\_bound}_{\strel}},
 \form{\code{expand}_{\strel}}, {\lbsea}.
We notice that, in this instantiation,
function \form{\code{init}_{\strel}} is an identity function;
function \form{\code{choose}_{\strel}} an open leaf in
a breath-first manner;
function \form{\code{prune\_out\_of\_bound}_{\strel}} (in line 8
of Algorithm \ref{algo.solved.sat}) checks whether
number boundaries of
an open leaf is beyond the bound \code{bound(n{,}m)}
where  \code{bound(n{,}m)} is presented
in Section \ref{sec.term}. If a leaf is
out\_of\_bound, it is marked as closed;
 function \code{expand} expands
a tree through a leaf
by firstly {\em unfolding} this leaf
into a set of normalized generalized equations and then
reducing these equations with {\em matching}.
Function \code{expand} is sketched as follows.
\[
\begin{array}{l}
\code{\bf foreach}~ \scge_i \in \unfoldsea((\utree{i},{\sge}_i)) ~ \code{\bf do}\\
\quad \code{match}(\scge_i) \\
\code{\bf end}
\end{array}
\]
%% In particular, in each iteration {\algoname}
%% first examines all {\sges} leaves using {\uo}
%% to detect a {\sat} leaf.
%% If there exists one, it returns with an appropriate counter-example.
%% Otherwise, it marks unsatisfiable leaves closed and
%% invoking {\oo} for {\unsat} checking.
%% For each remaining leaf,
%%  {\oo} over-approximates it prior to check it


==> complete.tex <==


\begin{lemma}[exponent of periodicity \cite{Koscielski:JACM:1996}]
If E is a word equation of the length d,  p is the
exponent of periodicity of a minimal solution of E,
then $p<2^{cd}$ with c is a constant.
\end{lemma}

\locsay{word equation without length constraints}

\begin{lemma}
number of boundary equation is greater than b,
then exponent of periodicity of solutions
of sub-tree a greater than G
\end{lemma}

\begin{lemma}
unfolding more than H then number of boundary equation is greater than b
\end{lemma}



\locsay{word equation with length constraints}
if unfold more than H then UNSAT on string constraints.
This implies that UNSAT for both string and arithmetic.

\subsection{Syntactic Termination}



restriction on arithmetic: Difference Constraints

Let
\form{x ={x_1, x_2, ..., x_N}}
be a set of variables ranging over
Z

Definition 3.
A formula \form{\phi(x)} is a difference bounds constraint
if it is equivalent to a finite conjunction of atomic propositions of the form
\form{x_i{-}x_j{\leq}a_{ij}},\form{1{\leq}i,j{\leq}N},
 \form{i{\neq}j}, where \form{a_{ij} {\in} Z}

if \form{x_i} and \form{x_j} are lengths of free variables.

restriction on arithmetic: Octagonal Constraints

\form{k_1v_i{+}k_2v_j{\leq}c} for any \form{v_i}, \form{v_j}
and \form{k_1,k_2{\geq}0}

\form{k_1v_i{+}k_2v_j{\geq}c} for any \form{v_i}, \form{v_j}
and \form{k_1,k_2{\leq}0}


==> fig-match.tex <==
\begin{figure*}[thb]
\begin{center}
%% \savespace
 \begin{minipage}{1\textwidth}
 \begin{frameit}\vspace*{-2.5mm}\savespace
\[
\renewcommand{\arraystretch}{1.1}
\begin{array}{c}
\match{CONSTs} \\
\form{\seppredF{\code{STR}}{u{,}0{,}r_u}} \text{ represents } c \qquad
\form{\seppredF{\code{STR}}{v{,}0{,}r_v}} \text{ represents } c  \\
\rho=[0/r_u,0/r_v] \quad \bases'{=} \{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}\rho ~|~ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \in \bases\} \\
\br'{=} \br {\setminus} \{\myit{i} ~|~ \FV(\myit{i}) {\subseteq} \{r_u,r_v\} \} \\
\code{match}(\satge{\bases'}{\boundaries{\setminus}\{r_u,r_v\}}{\br'}{Inv}) ~{\yields}~{\sge}
\\
\hline
\code{match}(\satge{\{\seppredF{\code{STR}}{u{,}0{,}r_u},\form{\seppredF{\code{STR}}{v{,}0{,}r_v}}\} {\cup} \bases}{\boundaries}{\br}{Inv}) ~{\yields}~{\sge}
\end{array}
\qquad
\renewcommand{\arraystretch}{1.1}
\begin{array}{c}
\match{CONST-VAR} \\
\form{\seppredF{\code{STR}}{u{,}0{,}r_u}} \text{ represents } c \qquad
\form{\seppredF{\code{STR}}{v{,}0{,}r_v}} \text{ represents a variable}  \\
\rho=[0/r_u] \quad \bases'{=} \{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}\rho ~|~ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \in \bases\} \\
\fresh ~v' \quad \br'{=} \br {\setminus} \{\myit{i} ~| \FV(\myit{i}) {\subseteq} \{r_u{,}r_v\} \} \\
{\sge} {=}\satge{\bases'}{\boundaries{\setminus}\{r_u\}}{\br'{\cup}\{r_v{\geq}0 \}}{Inv\subst{v'}{v}{\wedge}v'{=}c{\cdot}v}
\\
\hline
\code{match}(\satge{\{\seppredF{\code{STR}}{u{,}0{,}r_u},\form{\seppredF{\code{STR}}{v{,}0{,}r_v}}\} {\cup} \bases}{\boundaries}{\br}{Inv}) ~{\yields}~{\sge}
\end{array}
\]
\[
\renewcommand{\arraystretch}{1.1}
\begin{array}{c}
\match{VARs} \\
\form{\seppredF{\code{STR}}{u_i{,}0{,}r_u}},\form{\seppredF{\code{STR}}{u_{\dual{i}}{,}0{,}r_u}}  \text{ are dual of each another.}  \\
\rho=[0/r_u] \quad \bases'{=} \{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}\rho ~|~ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \in \bases\} \\
\bases''{=} \bases'{\cup} \{\seppredF{\code{STR}}{v'{,}0{,}r_v} \} \quad
\br'{=} \br {\setminus} \{\myit{i} ~|~ \FV(\myit{i}) {\subseteq} \{r_u\} \} \\
{\sge} {=}\satge{\bases''}{\boundaries{\setminus}\{r_u\}}{\br'{\cup}\{r_v{\geq}0 \}}{Inv{\wedge}u{=}c{\wedge}v{=}c{\cdot}v'}
\\
\hline
\code{match}(\satge{\{\seppredF{\code{STR}}{u_i{,}0{,}d_i},\form{\seppredF{\code{STR}}{u_{\dual{i}}{,}0{,}d_i}, \seppredF{\code{STR}}{t{,}l_t{,}r_t}}\} {\cup} \bases}{\boundaries}{\br}{Inv}) ~{\yields}~{\sge}
\end{array}
\]
\end{frameit}
 \end{minipage}
\caption{Matching Rules}\label{fig.sat.match}
\end{center}
\end{figure*}


==> fig-unfold-simpl.tex <==
\begin{figure}[thb]
\begin{center}
%% \savespace
 \begin{minipage}{1\textwidth}
 \begin{frameit}\vspace*{-2.5mm}\savespace
\[
\begin{array}{c}
\unf{\solvedF-CONST-SUCC}\\
{\unfoldsolve}(tr_1{=}tr_2 {\wedge} \pure) {\yields} L
\\
\hline
{\unfoldsolve}( c{\cdot}tr_1{=}c{\cdot}tr_2 {\wedge} \pure) ~{\yields}~L
\end{array}
~~
\begin{array}{c}
\unf{\solvedF-SMALL-L}\\
\seqs_1 {=} \seqs \subst{\semp}{\seppred{\code{STR}}{u{,}n}}\quad
\myit{I}_1{=}\myit{I} {\wedge}n{=}0 \quad
\subterm_1{=}\subterm {\wedge} u{=}\semp \quad L_1{=}\{tr_1{=}c{\cdot}tr_2 {\wedge} \seqs_1 {\wedge} \astart   {\wedge}  \myit{I}_1 {\wedge} \subterm_1\} \\
\seqs_2 {=}  \seqs\subst{c{\cdot}\seppred{\code{STR}}{u{,}n_1}}{\seppred{\code{STR}}{u{,}n}} \quad
 \myit{I}_2{=} \myit{I} {\wedge}n_1{=}n{-}1{\wedge}n{>}0
\quad  \subterm_2{=} \subterm \subst{u_1}{u}{\wedge} u_1{=}c{\cdot}u \quad \fresh~u_1\\
\hline
{\unfoldsolve}(\seppred{\code{STR}}{u{,}n}{\cdot}tr_1{=} c{\cdot}tr_2 {\wedge} \seqs {\wedge} \astart   {\wedge}  \myit{I} {\wedge} \subterm)  {\yields}L_1 {\cup} \{\seppred{\code{STR}}{u{,}n_1}{\cdot}tr_1{=}tr_2{\wedge}  \seqs_2 {\wedge}  \astart   {\wedge}  \myit{I}_2 {\wedge}\subterm_2\} \\
\end{array}
\]
\[
\begin{array}{c}
\unf{\solvedF-CONST-FAIL}\\
c_1{\not=} c_2
\\
\hline
{\unfoldsolve}( c_1{\cdot}tr_1{=}c_2{\cdot}tr_2 {\wedge} \pure) {\yields}\botF
\end{array}
~~
\begin{array}{c}
\unf{\solvedF-SMALL-R}\\
\seqs_1 {=} \seqs \subst{\semp}{\seppred{\code{STR}}{u{,}l{,}r}}\quad
\myit{I}_1{=}\myit{I} {\wedge}l{=}r \quad
\subterm_1{=}\subterm {\wedge} u{=}\semp \quad L_1{=}\{c{\cdot}tr_1{=}tr_2 {\wedge} \seqs_1 {\wedge} \astart   {\wedge}  \myit{I}_1 {\wedge} \subterm_1\} \\
\seqs_2 {=}  \seqs\subst{c{\cdot}\seppred{\code{STR}}{u{,}l_1{,}r}}{\seppred{\code{STR}}{u{,}l{,}r}} \quad
 \myit{I}_2{=} \myit{I} {\wedge}l_1{=}l{+}1{\wedge}l{<}r
\quad  \subterm_2{=} \subterm \subst{u_1}{u}{\wedge} u_1{=}c{\cdot}u \quad \fresh~u_1\\
\hline
{\unfoldsolve}(c{\cdot} tr_1{=} \seppred{\code{STR}}{u{,}l{,}r}{\cdot}tr_2 {\wedge}  \seqs {\wedge} \astart   {\wedge}  \myit{I} {\wedge} \subterm)  {\yields}
L_1{\cup}\{tr_1{=}\seppred{\code{STR}}{u{,}l_1{,}r}{\cdot}tr_2{\wedge}  \seqs_2 {\wedge}  \astart   {\wedge}  \myit{I}_2 {\wedge}\subterm_2\} \\
\end{array}
\]
\[
\begin{array}{c}
\renewcommand{\arraystretch}{1.1}
\unf{\solvedF-BIG}\\
\seqs_1 {=} \seqs \subst{u_1}{u_2}\quad
\myit{I}_1{=}\myit{I} {\wedge}l_1{=}l_2{\wedge}r_1{=}r_2 \quad
\subterm_1{=}\subterm {\wedge} u_1{=}u_2 \quad L_1{=}\{tr_1{=}tr_2 {\wedge} \seqs_1 {\wedge} \astart   {\wedge}  \myit{I}_1 {\wedge} \subterm_1\} \\
\seqs_2 {=} \seqs \subst{\seppred{\code{STR}}{u_2{,}l_2{,}r_2} {\cdot}\seppred{\code{STR}}{u_1{,}l_3{,}r_1}}{\seppred{\code{STR}}{u_1{,}l_1{,}r_1}} \quad
\myit{I}_2{=}\myit{I} {\wedge}l_1{=}l_2{\wedge}r_1{>}r_2 {\wedge} l_3{=}l_1{+}r_2 \quad
 \subterm_2{=}\subterm \subst{u_3}{u_1}{\wedge} u_3{=}u_2 {\cdot}u_1 \\
\seqs_3 {=} \seqs \subst{\seppred{\code{STR}}{u_1{,}l_1{,}r_1} {\cdot}\seppred{\code{STR}}{u_2{,}l_3{,}r_2}}{\seppred{\code{STR}}{u_2{,}l_2{,}r_2}} \quad
\myit{I}_3{=}\myit{I} {\wedge}l_1{=}l_2{\wedge}r_2{>}r_1 {\wedge} l_3{=}l_1{+}r_1 \quad
 \subterm_3{=}\subterm \subst{u_3}{u_2}{\wedge} u_3{=}u_2 {\cdot}u_1 \\
L_2{=}\{\seppred{\code{STR}}{s_1{,}l_3{,}r_1}{\cdot}tr_1{=}tr_2 {\wedge} \seqs_2 {\wedge} \astart   {\wedge}  \myit{I}_2 {\wedge} \subterm_2\} \qquad
 L_3{=}\{tr_1{=}\seppred{\code{STR}}{s_2{,}l_3{,}r_1}{\cdot}tr_2 {\wedge} \seqs_3 {\wedge} \astart   {\wedge}  \myit{I}_3 {\wedge} \subterm_3\} \\
\hline
{\unfoldsolve}(\seppred{\code{STR}}{u_1{,}l_1{,}r_1}{\cdot}tr_1{=} \seppred{\code{STR}}{u_2{,}l_2{,}r_2}{\cdot}tr_2 {\wedge} \seqs {\wedge} \astart   {\wedge}  \myit{I} {\wedge} \subterm) ~{\yields}~
L_1 {\cup} \{ L_2\} {\cup} \{ L_3\}
\end{array}
\]
\end{frameit}
 \end{minipage}
\caption{Unfolding Rules for {\satsolved}}\label{fig.sat.simple.unfold}
\end{center} \savespace
\end{figure}


==> impl.tex <==
We have implemented the proposed decision procedure using OCaml.


==> motivate.tex <==

\subsection{Overview}
\paragraph{A Generic Satisfiability Procedure}

Normalized Formula




\subsection{Illustrative Examples}


==> multi-wordeq.tex <==
\label{sec.mul.eq}
We first show a reduction from
a formula with
multiple word equations to
an equivalent formula with single word equation.
We adapt the approach presented in \cite{khmelevski1976equations}
to reduce multiple word equations.
This approach is summarized in the following lemmas.

\begin{lemma}[1.28 \cite{khmelevski1976equations}]
For any system of word equations in \form{n}
unknowns it is possible to construct a word equation
in \form{n} unknowns which is equivalent to the system.
\end{lemma}

The above lemma was proven based on the following lemma.
\begin{lemma}[\cite{khmelevski1976equations}]\label{lemma.eqs}
Suppose that \form{X_1}, \form{X_2}, \form{Y_1} and
\form{Y_2} are words in \form{\alphabet^*}
and
\[
 \form{X_1{\cdot}c_1{\cdot}X_2{\cdot}X_1{\cdot}c_2{\cdot}X_2~{=}~Y_1{\cdot}c_1{\cdot}Y_2{\cdot}Y_1{\cdot}c_2{\cdot}Y_2}
\]
 where \form{c_1} and \form{c_2}
are distinct characters in \form{\alphabet}.
Then, \form{X_1{=}Y_1} and  \form{X_2{=}Y_2}.
\end{lemma}


==> sat-algo-simp.tex <==
 %% \begin{figure}[tbh]
 %% \begin{center}
 %% \begin{minipage}{0.98\textwidth}
 % \begin{frameit}

 \begin{algorithm}[t]
%%\begin{procedure}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$\ind$} \Output{{\sat} or {\unsat}}
   $i {\leftarrow} 0 $; %% $\sstate^{comp} {\leftarrow} \{ \}$;
  $\ind_0 {\leftarrow} \code{indize}(\ind)$; %% \tcc*{label}
   $\utree{0} {\leftarrow} \{ \ind_0 \}$ \tcc*{initialize}
 \While { $\true$ }
 {
    (\code{is\_sat},\utree{i}) {$\leftarrow$} \code{\uosolve}(\utree{i})  \tcc*[r]{check {\sat}}
   {\bf if} {\code{is\_sat}} {\bf then }
   {\Return{${\sat}$} \tcc*{\sat}}
   \Else{
     $\utree{i} {\leftarrow} \code{\oosolve}(\utree{i})  $ \tcc*[r]{prune {\unsat}}
      $ \utree{i}  {\leftarrow} \code{\lbsolve}(\utree{i}) $ \tcc*[r]{cyclic proof}
     %% $ \sstate  {\leftarrow} \code{\fix}(\sstate, \sstate^{bud}) $ \tcc*[r]{detect fixpoint}
     {\bf if} {\code{is\_closed}(\utree{i})} {\bf then } {\Return{{\unsat} }\tcc*{\unsat}}
	 \Else{
       $\ind_i {\leftarrow} \code{dfs\_choose}(\utree{i})  $ \;
	   $ i {\leftarrow} i{+}1 $ \;
       $ \utree{i}  {\leftarrow} {\unfoldsolve}(\ind_i) $\;
  %%   $ \sstate  {\leftarrow} (\sstate \setminus \{\ind_i\}) \cup \sstate_i $\;
  %%   $ \sstate^{comp}  {\leftarrow} \sstate^{comp} \cup \{\ind_i\} $\;
      }
   }
 }
 \caption{Procedure {\satsolved}}\label{algo.solved.sat}
\end{algorithm}
%\savespace
%%\end{procedure}


==> sat-algo.tex <==
 %% \begin{figure}[tbh]
 %% \begin{center}
 %% \begin{minipage}{0.98\textwidth}
 % \begin{frameit}

 \begin{algorithm}[t]
%%\begin{procedure}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$\sge_0(n,m)$} \Output{{\sat} or {\unsat}}
  %% \Function{}{}
   $i {\leftarrow} 0 $;
   %% $\sge_0(n,m) {\leftarrow}  \code{reduce}(\pure)$ \tcc*{reduce}
   $\utree{0} {\leftarrow} \{ \sge_0 \}$ \tcc*{initialize}
 \While { $\true$ }
 {
    (\code{is\_sat},\utree{i}) {$\leftarrow$} \code{\uosea}(\utree{i})  \tcc*[r]{check {\sat}}
   {\bf if} {\code{is\_sat}} {\bf then }
   {\Return{${\sat}$} \tcc*{\sat}}
   \Else{
     $\utree{i} {\leftarrow} \code{\oosea}(\utree{i})  $ \tcc*[r]{prune {\unsat}}
      $ \utree{i}  {\leftarrow} \code{\lbsea}(\utree{i}) $ \tcc*[r]{isomorphic}
     $\utree{i} {\leftarrow} \code{prune\_out\_of\_bound}(\utree{i}{,}n{,}m)$ \;
     {\bf if} {\code{is\_closed}(\utree{i})} {\bf then } {\Return{{\unsat} }\tcc*{\unsat}}
	 \Else{
           \ForEach{${\sge}_i$ $\in$ \code{choose\_bfs}(open\_leaves(\utree{i})) }{
             \ForEach{${\scge}_i$ $\in$  {\unfoldsea}(\utree{i},${\sge}_i$)}{
               %% ${\scge}_i {\leftarrow} \code{unfold}(\utree{i},{\sge}_i)$\;
               %% \Begin{
               %%     \Switch{${\scge}_i$}{
               %%       \Case{1}{
               %%         $ {\sge'}_i {\leftarrow} \code{match}({\scge}_i)$;
               %%         $ \utree{i} {\leftarrow} \algoname({\sge'}_i) $
               %%       }
               %%      }
               %% }
                $ \utree{i}  {\leftarrow} \code{match}({\scge}_i) $\;
              }
          }
      %% ${\sge}_i {\leftarrow} \code{choose\_bfs}(\utree{i})  $\;
	   $ i {\leftarrow} i{+}1 $ \;
      }
   }
 }
 %%\EndFunction
 \caption{Procedure {\algoname}}\label{algo.s2.sat}
\end{algorithm}
%\savespace
%%\end{procedure}


==> sat.tex <==
\input{algo}


\paragraph{Under-Approximating}
Function {\uosea} only considers open leaves in the decidable fragment
%% {\simpleF}.
 {\solvedF}.
It examines a generalized equation \form{\sge} stored
 in an open leaf through two steps.
 First, it
 checks whether \form{\sge} could be syntactically
reduced into a {\solvedF} formula
  or not. After that it constructs  an equivalent
 {\solvedF} formula of {\sge} and invokes \form{\satsolved} to discharge
 the  {\solvedF} formula.
%% A generalized equation {\sge} with the following components
%% \satge{\bases}{\boundaries}{\br}{Inv}
%%  is in {\simpleF}
%% if
%% all its variable bases are empty.

Let \form{\sge\satge{\bases}{\boundaries}{\br}{Inv}} be  a generalized equation.
There are two cases where {\sge} may be reduced
 to an equivalent {\solvedF} formula.
The first case is
where all variable bases in \form{\bases} are empty.
Function {\uosea} constructs
the conjunction
\form{\br{\wedge}Inv} as an equivalent base formula
of {\sge}
We recap that the conjunction \form{\br{\wedge}Inv}
is always in the {\simpleF} logic. It is easy to show that
{\sge} is satisfiable iff \form{\br{\wedge}Inv} is satisfiable.
%% {\uo} checks whether \form{\br{\wedge}Inv} is satisfiable
%% using \form{\satsolved(\br{\wedge}Inv)}.
%% We notice that the conjunction \form{\br{\wedge}Inv}
%% is always in the {\simpleF} logic.
%%
%% In the following, we show how {\uosea} identifies and discharges a 
%% {\solvedF} generalized equation {\sge} in general.
%% with components \satge{\bases}{\boundaries}{\br}{Inv}.
%%
%% First, it reverses {\sge}
%% back to an equivalent string formula \form{\pure_i}, if possible.
%% Second, if \form{\pure_i} is in the base logic, i.e. in {\solvedF}
%% fragment, it invokes \form{\satsolved(\pure_i)}
%% for satisfiability checking.
The second case is where  each string variable is presented by at most
 one pair of dual non-empty variable bases
 in \form{\bases}
 and arithmetic is as described for {\solvedF}.
Function {\uosea constructs the base formula \form{\pure_i} as follows.
\begin{enumerate}[topsep=1pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item As satisfiability of empty bases are encoded in \form{Inv}, only  non-empty bases
need to be considered.
Let \form{\bases_1} be a subset or equal of \form{\bases}
which contains all non-empty bases.
\item For each dual of two bases \form{\seppredF{\code{STR}}{u{,}l_i{,}r_i}}
and \form{\seppredF{\code{STR}}{\dual{u}{,}l_j{,}r_j}} in \form{\bases_1},
if \form{l_i{=}l_j} and \form{r_i{=}r_j} then drop the base \form{\seppredF{\code{STR}}{\dual{u}{,}l_j{,}r_j}}. Let \form{\bases_2} be the remaining bases.
\item Let \form{\theta{=} {\circ }\{\subst{u}{\dual{u}} \mid u{,}\dual{u} {\in} \bases_2 \text{ and } \text{are dual.} } \}.
\item Let \form{tr_1{=}\semp}, and \form{d_i{=}0}. Repeat the following process:
\begin{enumerate}[topsep=0pt,itemsep=0ex,partopsep=0ex,parsep=0ex]
\item  Let \form{\seppredF{\code{STR}}{u_i{,}l_i{,}r_i}}
be in \form{\bases_2} where \form{l_i{=}d_i}. If can not find such a base, stop.
\item \form{tr_1{=}tr_1{\cdot}u_i}
\item \form{\bases_2{=}\bases_2 \setminus \{ \seppredF{\code{STR}}{u_i{,}l_i{,}r_i} \}}
 \item
 \form{d_i{=} r_i}
\end{enumerate}
\item  Let \form{tr_2{=}\semp}, and \form{d_i{=}0}. Repeat the similar steps 4(a)-4(d) above
to construct \form{tr_2}.
\item If \form{\bases_2} is empty afterward then return the formula
\saveone\[\saveone
 \form{\pure_i{\equiv}(tr_1{=}tr_2 {\wedge} \br {\wedge} Inv)\theta}
\] Otherwise, there is  no base formula for {\sge}.
\end{enumerate}
It is easy to show that {\sge} has a solution {\sgesol} with a pair
(\form{\sstack}, \form{\istack}) iff \form{\pure_i} has a solution
(\form{\sstack}, \form{\istack}).


\paragraph{Over-Approximating}
Let \form{\sge\satge{\bases}{\boundaries}{\br}{Inv}} be a generalized equation.
Function {\oo} checks whether {\sge} is unsatisfiable
through one of the two following procedures.
\begin{enumerate}
\item For each boundary \form{d_i {\in} \boundaries},
if (i) there exist two {\em constant} bases
\form{\seppredF{\code{STR}}{u{,}l_u{,}r_u}}
and \form{\seppredF{\code{STR}}{v{,}l_v{,}r_v}} in \form{\bases}
such that \form{l_u{=}d_i} and \form{l_v{=}d_i},
and (ii) these two based represent to two different characters
 (e.g., \form{c_1}, \form{c_2} \form{c_1{\neq}c_2}),
 then {\sge} is unsatisifiable.
\item if \form{\satsolved(\br {\wedge}Inv)} is 
 unsatisfiable then so is {\sge}.
\end{enumerate}


%% replace all constants with the same character \cite{Makanin:math:1977},
%% if unsat then unsat

\paragraph{Linking Back}
Function {\lbsea} links an open leaf back to an equal inner node.
We define that
two generalized equations are equal if they become isomorphic by
some substitutions of names of boundaries and variable bases.
This function is implemented similarly to the function {\lbsolve} in
subsection \ref{solved.algo}.
We omit the details.

\paragraph{Unfolding}
\input{sat-unfold}

\paragraph{Matching}
\input{sat-match}

